Learning Electromagnetic Metamaterial Physics With ChatGPT

Large language models (LLMs) such as ChatGPT, Gemini, LlaMa, and Claude are trained on massive quantities of text parsed from the internet and have shown a remarkable ability to respond to complex prompts in a manner often indistinguishable from humans. For all-dielectric metamaterials consisting of unit cells with four elliptical resonators, we present a LLM fine-tuned on up to 40,000 data that can predict the absorptivity spectrum given a text prompt that only specifies the metasurface geometry. Results are compared to conventional machine learning approaches including feed-forward neural networks, random forest, linear regression, and K-nearest neighbor (KNN). Remarkably, the fine-tuned LLM (FT-LLM) achieves a comparable performance across large dataset sizes with a deep neural network. We also explore inverse problems by asking the LLM to predict the geometry necessary to achieve a desired spectrum. LLMs possess several advantages over humans that may give them benefits for research, including the ability to process enormous amounts of data, find hidden patterns in data, and operate in higher-dimensional spaces. This suggests they may be able to leverage their general knowledge of the world to learn faster from training data than traditional models, making them valuable tools for research and analysis.

==> scratch_pad.tex <==
% Potential alternative structure for the introduction, from this point forward. 
% 1) What are LLMs?  "Recently LLMs have emerged as a type of foundation model that is focused on modeling human language, and by extension reasoning."  

% 2) Why are LLMs Interesting?  "LLMs possess several exciting properties.  (i) they seem to possess/remember broad knowledge about the world that has been provided to them in their training set,  (ii) they can perform basic reasoning about the information provided to them in their training set.  This reasoning is often provided in the form of output text generated by the model, in response to queries that are provided to the model as input.  For example, LLMs can answer basic questions about science, or even perform logical reasoning, such as performing basic mathematics (e.g., addition, integration, differentiation).  (iii) lastly, the LLMs can often explain their reasoning, providing some level of explainability/interpretability.  

% 3) How Might LLMs be used in AEM.  "In this work we hypothesize that LLMs, such as ChatGPT, may be able to leverage these capabilities to reason about physical systems with far less training data than existing DNN-based models.  (Explain why)

% Note. I briefly investigated "What is the difference between LLMs and FoMos", according to the internet.  First, these are somewhat vague concepts, which are evolving quickly.  With that in mind, there seemed to be some concensus that LLMs can be thought of as a particular type of foundation model that has been fine-tuned/specialized for human language, and can form the "backbone" for various models that solve problems in natural language processing (e.g., spam detection, sentiment analysis, or question answering, etc). 
